On the growth rate of polyregular functions

We consider polyregular functions, which are certain string-to-string functions that have polynomial output size. We prove that a polyregular function has output size $\mathcal O(n^k)$ if and only if it can be defined by an MSO interpretation of dimension $k$, i.e. a string-to-string transformation where every output position is interpreted, using monadic second-order logic MSO, in some $k$-tuple of input positions. We also show that this characterization does not extend to pebble transducers, another model for describing polyregular functions: we show that for every $k \in \{1,2,\ldots\}$ there is a polyregular function of quadratic output size which needs at least $k$ pebbles to be computed.

==> conclusion.tex <==
%!TEX root = main.tex

\section{Conclusion and perspectives}

\paragraph{Pebble minimization in special cases.}

As mentioned at the end of the introduction, the pebble and growth rate
hierarchies coincide for both marble transducers~\cite{Marble} and
comparison-free pebble transducers~\cite{NguyenNP21}. The restrictions that
these two machine models impose on pebble transducers seem at first sight
orthogonal, so it is intriguing that both lead to a \enquote{pebble
  minimization} theorem despite its failure in the general case.

However, marble transducers are actually \enquote{almost comparison-free}: they
only need to compare their head with the second-topmost pebble on the stack.
This condition, which has been called \enquote{invisible
  pebbles}~\cite{InvisiblePebbles}, is violated by the pebble transducers that
compute the map power and $k$-zebra functions. This leads us to conjecture that
transducers with invisible pebbles enjoy a pebble minimization property.

Another special case where pebble minimization works is when the output alphabet
is unary (but the input alphabet can be arbitrary),
cf.~Remark~\ref{rem:unary-output}. We also believe that it applies to
polyregular functions with unary input and arbitrary output; this could
hopefully follow from a \enquote{closed-form description} of such functions,
similar to \cite[Theorem~9.2]{NguyenNP21}.

\tito{More relationships between growth rates and machine models? For instance,
  a conjecture: if a composition of TWT (actually a very canonical tree
  transduction class!) is string-to-string and has polynomial size increase,
  then it is polyregular. And if this is true: are compositions of TWT with
  $n^{O(1)}$ growth the \enquote{right} notion of polyregular tree functions?
refer to the proof of Theorem~\ref{thm:linear-polyregular}}

\tito{The usual way to automatically generate new questions: what about the
  aperiodic / first-order case? Also, what does the Seed Lemma tell us about the
  notion of origin semantics for polyregular functions? (Something concrete:
  given an \mso query + \mso-defined ordering on selected tuples, can we decide
  whether they are FO-definable?)}


==> factorization-forests.tex <==
\subsection{Factorization trees and their skeletons}
\label{sec:factorization-forests}
The second ingredient that will be used in the  proof of the Seed Lemma is the  Factorization Forest Theorem. This theorem    tells us that each word admits a nested decomposition with respect to a given semigroup homomorphism, so that the nesting depth is bounded and at each nesting step the decomposition is very simple. 


In this paper, when talking about trees, we mean finite node-labelled  rooted trees which are sibling ordered, i.e.~for every node there is a linear order on its children. Also, every set of trees that we will consider will have bounded depth. The \emph{yield} of a tree is the word obtained by reading the leaves of the tree from left to right.
A  \emph{factorization tree} for a semigroup homomorphism $h : \Sigma^+ \to S$  is defined to be a tree where:
\begin{enumerate}
    \item leaves are labelled by letters from $\Sigma$, while internal nodes (i.e.~non-leaves) are labelled by semigroup elements from $S$;
    \item every internal node is labelled by the value of $h$ on the  yield of its subtree;
    \item if an internal node has more than two children, then all of these children have the same label, and this label is an idempotent in the semigroup $S$.
\end{enumerate} 
Define the  \emph{height}  of a tree to be the maximal number of edges that can be found on a root-to-leaf path. Here is a picture of a factorization tree of height 4:
\mypic{1}

The Factorization Forest Theorem says that if a semigroup homomorphism is fixed, then every word can be obtained as the yield of some factorization tree of bounded height. 
\begin{theorem}
    [Factorization Forest Theorem] Let $h : \Sigma^+ \to S$ be a semigroup homomorphism  with $S$ finite. There is some $m \in \set{1,2,\ldots}$ such that every   word in $\Sigma^+$ is the yield of some factorization tree  of height at most $m$. 
\end{theorem}
The theorem was originally proved by Imre Simon~\cite[Theorem 6.1]{simonFactorizationForestsFinite1990}, and an  optimal bound for the number $m$ is $3  |S| -1$, see~\cite[Theorem 2]{kufleitner2008}.

\newcommand{\parent}{\mathrm{parent}}


\paragraph*{Skeletons.} Consider a query recognized by a semigroup homomorphism  $h : \Sigma^+ \to S$. Suppose that we are given factorization tree for this homomorphism, with a distinguished tuple of  leaves indexed by the free variables of the query. (We use the name \emph{pointed factorization tree} for such an object.)  From a pointed factorization tree we can obtain a pointed word, by ignoring the internal nodes and just looking at the yield. We will  show that whether or not (the pointed word corresponding to) a pointed factorization tree satisfies a query  can be inferred from  information about the distribution of the distinguished leaves. This information is  called the skeleton, and is defined as follows. 

Define the \emph{closure} of a set of nodes in a tree  to be the least set which contains these nodes  and which is closed under taking parents, leftmost siblings, and rightmost siblings.  (The leftmost sibling is the one that does not have a previous sibling, likewise we define rightmost siblings.) If the height of the tree is assumed to be bounded, and the number of distinguished nodes is also bounded, then the size of the closure is bounded, because the closure contains at most three nodes for each ancestor of a distinguished node. For a tree with distinguished leaves (think of a  pointed factorization tree), define its \emph{skeleton} to be the tree restricted to the closure of the distinguished leaves, plus the information about  which nodes of the closure were consecutive siblings in the original tree (such nodes are said to be \emph{linked} in the skeleton). Here, the {consecutive sibling} relation  is the partial function that maps a node to its next sibling, if it exists.   We view the closure also as a tree with  distinguished leaves, the same distinguished leaves as in the original tree.  Here is a picture of a tree with distinguished leaves   and its skeleton:
\mypic{2}
In the picture of the skeleton, the dotted lines indicate missing pieces of the original tree, which separate siblings that are not consecutive. If the original tree was a factorization tree, as will be the case in our intended application, then dotted lines represent multiple copies of an idempotent, since dotted lines require at least 5 siblings to appear, which is more than the threshold 3 required to have an idempotent label. 

\begin{lemma}[Skeleton]\label{lem:reading-forest} For every pointed factorization tree (with respect to a homomorphism that recognizes $\varphi$), whether or not the corresponding pointed word satisfies $\varphi$ depends only on the skeleton. 
\end{lemma}
\begin{proof}
    In order to know if $\varphi$ is true in the corresponding pointed word, we need to know: (a) the labels and ordering of  the distinguished leaves; and (b) the value of the semigroup homomorphism on infixes of the yield word that are between two consecutive distinguished leaves (or the endpoints of the word). It is not hard to see that this information  can be read from the skeleton. 
    % For (a) there is nothing to do, since the skeleton stores the labels and the relative ordering on the distinguished nodes. To see how (b) can be recovered from the skeleton, one uses the labels in the skeleton to recover all of the semigroup elements that correspond to subtrees that separate two consecutive distinguished leaves. The main observation is that if we have two consecutive siblings in the skeleton which are not linked (i.e.~in the original tree they were not consecutive), then we know that missing part of the tree between the siblings was an several copies of a known idempotent, and therefore the value of the missing part under the homomorphism can be determined by looking at the skeleton.
\end{proof}

 

==> lower-bound.tex <==

In this note, we try to argue that a 2-pebble transducer cannot recognize the Ga\"etan function 
\begin{align*}
g(a^{n_1}b \cdots a^{n_k}b) \qquad \mapsto \qquad 
(a^{n_1}b)^k \cdots (a^{n_k}b)^k.
\end{align*}
We view an input string as tree of depth 2 as explained in the following picture:

For a threshold $\omega \in \set{1,2,\ldots}$ we say that two numbers are $\omega$-similar if either: (a) both numbers are equal and smaller than $\omega$; or (b) both numbers are at least $\omega$, and congruent modulo $\omega$. Define the \emph{address} of a position  $x$ in an input word  to be the following numbers: 
\begin{align*}
\myunderbrace{\text{number of $b$ positions $\le x$}}{d}
\end{align*}

We say that two nodes in a tree of depth 2 are  $\omega$-similar if the following conditions all hold:
\begin{enumerate}
    \item both nodes have the same depth;
    \item if both nodes have depth $\ge 1$, i.e.~both are not the root, then 
\end{enumerate}

Fix for the rest of this note a 2-pebble transducer. Define a \emph{block} in an input word to be a maximal set of consecutive $a$'s.  For a position $x$ in an input word define its \emph{global address} to be the pair of numbers
\begin{quotation}
    (number of $b$'s before $x$, number of $b$'s after $x$).
\end{quotation}
Likewise we define the \emph{local address}, 



\begin{lemma}
    There exists a number $\omega \in \set{1,2,\ldots}$, which depends on the fixed pebble transducer, such that the following holds. Let $t$ be an input tree of depth 2 where every node has a number of children that is divisible by $\omega$ (such trees will be called \emph{$\omega$-smooth}). If $\alpha$ and $\beta$ are two configurations that are $\omega$-equivalent, then either both or none appear in the run of the pebble transducer on $t$.
\end{lemma}
Let $\omega \in \set{1,2,\ldots}$ be some large number. We also assume that $\omega$ is a factorial, and as a consequence $m^\omega$ will be an idempotent for every element $m$ of a sufficiently small finite monoid $M$, including the monoid which describes the pebble movement of the fixed pebble transducer. 
We say that an input word 
\begin{align*}
a^{n_1}b \cdots a^{n_k}b 
\end{align*}
is \emph{hard} if all of the numbers $n_1,\ldots,n_k$ and $k$ are nonzero multiples of $\omega$, and also all of these numbers are distinct. For hard input words, the movement of pebble 1 (the main pebble, at the bottom of the stack) is going to follow a very regular patter, which consists roughly of a constant number of sweeps through the input word, with a constant number of sub-sweeps for each block of $b$'s. 

Define a 1-configuration to be a configuration of the pebble automaton where only 1 pebble is present, the remaining configurations are 2-configurations. For a 1-configuration and a fixed input word, define its \emph{2-subcomputation} to be the 1-configuration together with all subsequent 2-configurations, until (but not including) the nearest 1-configuration. Define the \emph{partial output} of a 1-configuration in a given input word to be the output that is produced during the  2-subcomputation that corresponds to this 1-configuration.

In the following lemma, and in all proofs afterward, a \emph{block} in a word over the alphabet $\set{a,b}$ is defined to be a maximal infix of the form $a^*b$. We will consider blocks both in the input and in the output strings. 

In the following, we will use the name  \emph{affine function} for any function of type $\Nat^d \to \Nat$ of the form
\begin{align*}
(a_1,\ldots,a_d) \mapsto \lambda + \lambda_1 a_1 + \cdots + \lambda_d a_d.
\end{align*}
The numbers $\lambda,\lambda_1,\ldots,\lambda_d$, which are called \emph{coefficients} of the affine function, are assumed be in $\Nat$, since otherwise the function would produce outputs outside~$\Nat$.  We will be interested in affine functions where all coefficients are bounded by some constant $\ell \in \set{0,1,\ldots}$. The following lemma shows that the sizes of certain \mso definable sets can be described by such  affine functions. 


\begin{lemma}\label{lem:affine-mso}
    For every \mso definable binary relation $\varphi(x,y)$ on  positions in strings over $\set{a,b}^*$,  there is a number $\omega \in \set{1,2,\ldots}$ with the following property. If $x$ is a position in an input word 
    \begin{align*}
    w = a^{n_1}b \cdots a^{n_k}b \qquad 
    \myunderbrace{\text{such that all numbers $k,n_1,\ldots,n_k$ are divisible by $\omega$}}{input words that satisfy this condition are called $\omega$-hard},
    \end{align*}
    then the number of positions $y$ which satisfy $\varphi(x,y)$ 
    is obtained by applying some affine functions, with coefficients of size at most $\ell$, to the following numbers:
    \begin{align*}
        \myunderbrace{n_1,\ldots,n_\ell}{lengths of a \\ \scriptsize constant number \\
        \scriptsize of first blocks}
        \qquad 
        \myunderbrace{n_{x[1]-\ell},\ldots,n_{x[1]+\ell}}{lengths of a \\ \scriptsize constant number \\
        \scriptsize of blocks around $x[1]$}
        \qquad 
        \myunderbrace{n_{k-\ell},\ldots,n_{k}}{lengths of a \\ \scriptsize constant number \\
        \scriptsize of last blocks}
        \qquad
        \myunderbrace{x[2], -x[2]}{position in\\ \scriptsize block $x[1]$}.
        \end{align*}
\end{lemma}
\begin{lemma}
    There is a constant $\ell \in \set{1,2,\ldots}$, which depends only on the 2-pebble automaton, such that the following holds. 
Let 
\begin{align*}
w = a^{n_1}b \cdots a^{n_k}b
\end{align*}
be a hard input word, and consider the partial output that is produced by the children of some 1-configuration $\alpha$. Then the length of each block  differs by at most $\ell$ from some number on the following  list:
    \begin{align*}
    \myunderbrace{n_1,\ldots,n_\ell}{lengths of a \\ \scriptsize constant number \\
    \scriptsize of first blocks}
    \qquad 
    \myunderbrace{n_{\alpha[1]-\ell},\ldots,n_{\alpha[1]+\ell}}{lengths of a \\ \scriptsize constant number \\
    \scriptsize of blocks around $\alpha[1]$}
    \qquad 
    \myunderbrace{n_{k-\ell},\ldots,n_{k}}{lengths of a \\ \scriptsize constant number \\
    \scriptsize of last blocks}
    \end{align*}
\end{lemma}
\begin{proof}
    Consider the binary relation $\varphi$ between configurations, which relates a pair of configurations $(\alpha,\beta)$  in the same input string  if $\beta$ is a child configuration of $\alpha$, there is exactly one letter $b$ that is produced between $\alpha$ and $\beta$, and  the output produces by $\beta$ is $a$ (unfortunate notation). If we fix the input string and $\alpha$,  then  we from Lemma~\ref{lem:affine-mso} that the size of the set
    \begin{align}\label{eq:child-configurations}
    \set{ \beta : \varphi(\alpha,\beta)}
    \end{align}
    is an affine combination  of the numbers on the list from the statement of this lemma, plus also the numbers $\alpha[2]$, $-\alpha[2]$ and $k$, which uses coefficients that are bounded by some constant $\omega$ that depends only on the fixed pebble transducer. We also know that the size of the set~\eqref{eq:child-configurations} is one of the numbers $n_1,\ldots,n_k$, because of the way that the transducer works. 
    \begin{align*}
    n_i = 
    \end{align*}
    
    and  with the coefficients of the linear combination depending only on the \mso theory of $\alpha$ with respect to some constant quantifier rank (that depends only on the transducer and not on $\alpha$ or the input). Let $N \in \set{1,2,\ldots}$ be the maximal absolute value of these coefficients. Since our transducer computes Gaetan's function, it follows that the size of the set~\eqref{eq:child-configurations} is one of the number $n_1,\ldots,n_k$. If we assume that all of these numbers 

    Let $\alpha$ be the 1-configuration in question, and let $\beta_1,\ldots,\beta_m$ be the child configurations of $\alpha$ which output $b$'s. We claim that if $\beta_i$ is such that 
\end{proof}

\begin{lemma}
    Let $\beta$ be a configuration that appears in a run over some hard input, and which outputs $b$. Let $i,j \in \set{1,\ldots,k}$ be the block numbers that contain both pebbles (if $\beta$ is a configuration with just one pebble, then $i=j$).  Then the output block of $\beta$ 
    has length that differs by at most $\ell$ from some number on this list:
    \begin{align*}
    \myunderbrace{n_1,\ldots,n_\ell}{left blocks}
    \qquad 
    \myunderbrace{n_{i-\ell},\ldots,n_{i+\ell}}{blocks close to $i$}
    \qquad 
    \myunderbrace{n_{j-\ell},\ldots,n_{j+\ell}}{blocks close to $j$}
    \qquad 
    \myunderbrace{n_{k-\ell},\ldots,n_{k}}{middle blocks}
    \end{align*}
\end{lemma}

% Before proving the lemma, we use it to prove that our fixed 2-pebble transducer cannot compute the function $g$. Indeed, consider all 1-configurations in the run of this transducer on some hard input word. We partition 1-configurations into \emph{central configurations} (those where pebble 1 satisfies the assumptions of the lemma, i.e.~it has at least $\ell$ occurrences of $b$ to the left and right), and the remaining ones which are called \emph{non-central}. By the lemma, the output produced in central configurations and their 2-subcomputations will have a number of $b$'s which is linear in the number of 
% By the lemma, the number of $b$'s that is output in 2-subcomputation 

% for the output that is produced if we start the automaton in configuration $(q,x)$ in an input word $w$, and we wait until 

% A configuration of the two-pebble automaton is either $q(x)$ or $q(x,y)$, where $q$ is a control state and $x,y$ are pebble positions. 


==> monad.tex <==
\section{Query algebras}
\label{sec:monad}
In this appendix,  we take the proofs from Section~\ref{sec:seed-lemma}, and recast their conclusions in a more algebraic terminology. This terminology uses an algebraic structure, called a \emph{query algebra}, which is meant to be the analogue of semigroups for pointed words.
For conciseness, we define query algebras as a special case of algebras in a suitably chosen monad. Since the results of this appendix are not used elsewhere in the paper,  we present the definitions assuming that  the reader is familiar with monads and their algebras, and we only give sketches of the proofs. For more details about monads, see~\cite[Section 4]{bojanczyk_recobook}. 


\paragraph*{An monad for pointed words.}
Let us write $\queryalg X \Sigma$ for the set of pointed words where the variables are $X$ and the alphabet is  $\Sigma$. For a fixed set of variables $X$, the operation  $\Sigma \mapsto \queryalg X \Sigma$ can be equipped  with the structure of a monad (in the category of sets), as follows\footnote{In the special case where $X$ has one variable, this monad was  studied in~\cite[Section 8]{bojanczykRecognisableLanguagesMonads2015}.}.  The structure of the monad $\queryalg X$ consists  of three families of functions
\begin{align*}
\myunderbrace{\queryalg X f : \queryalg X \Sigma \to \queryalg X \Gamma}{indexed by functions\\
\scriptsize $f : \Sigma \to \Gamma$}
\qquad
\myunderbrace{\mathrm{unit}_X : \Sigma \to \queryalg X \Sigma}{indexed by sets $\Sigma$}
\qquad
\myunderbrace{\mathrm{flat}_X : \queryalg X \queryalg X \Sigma \to \queryalg X \Sigma}{indexed by sets $\Sigma$}.
\end{align*}
In all of three families of functions described above, the alphabets $\Sigma$ and $\Gamma$ range over possibly infinite sets.
The first family describes how a function $f$ on alphabets can be extended to a function on pointed  words; the extended function  simply changes the labels in the input pointed word according to $f$.  The second family describes how an input letter can be seen as a pointed word, this pointed word has a unique position labelled by the letter, and all variables point to this unique position. The third family describes how a pointed word of pointed words can be flattened to a pointed word, this operation is explained in the following picture:
\mypic{7}
In the flattened pointed word, variable $x \in X$ points to the following position: follow variable $x$ in the original pointed word of pointed words, yielding a pointed word, and in that pointed word follow variable $x$ again.
One can easily check that the functions described above satisfy the axioms of a monad, see e.g.~\cite[Section 4.1.1]{bojanczyk_recobook} for a list of these axioms. We call this the \emph{monad of $X$-pointed words}, there is one monad for every choice of $X$.

Define a  \emph{query algebra over variables $X$} to be an Eilenberg-Moore algebra for the monad $\queryalg X$, see~\cite[Definition 4.3]{bojanczykRecognisableLanguagesMonads2015}. Such a query algebra consists of  an underlying set $A$ together with a \emph{multiplication operation} of type $\queryalg X A \to A$, subject to certain natural axioms. 
% subject to the following two axioms: (i) if we apply the multiplication operation to the unit of $a \in A$, then we get $a$; and (ii) multiplication is compatible with flattening in the sense that the following diagram commutes:
% \[
%     \begin{tikzcd}[column sep=4cm]
%         \queryalg X \queryalg X A 
%         \ar[r,"\queryalg X\text{(multiplication in $A$)}"]
%         \ar[d,"\text{flattening}"']
%         & \queryalg X A
%         \ar[d,"\text{multiplication in $A$}"] \\
%         \queryalg X A
%         \ar[r,"\text{multiplication in $A$}"']
%          & A
%     \end{tikzcd}
%     \]
An important example of a query algebra is $\queryalg X \Sigma$, for any set $\Sigma$, equipped with flattening as the multiplication operation; algebras of this form are called \emph{free}.
A \emph{homomorphism} of two  query algebras over the same variables $X$ is defined to be a function $h : A \to B$ between their underlying sets which is compatible  with multiplication in the sense that the following diagram commutes:
\[
    \begin{tikzcd}[column sep=4cm]
        \queryalg X A 
        \ar[r,"\text{multiplication in $A$}"]
        \ar[d," \queryalg X  h"']& A
        \ar[d,"h"] \\
        \queryalg X B
        \ar[r,"\text{multiplication in $B$}"']
         & B
    \end{tikzcd}\]



 A query with variables $X$ and input alphabet $\Sigma$ is the same thing as a subset of a free algebra $\varphi \subseteq \queryalg X \Sigma$. Such a query is said to be \emph{recognized} by a homomorphism of query algebras 
\begin{align*}
h : \queryalg X \Sigma \to A
\end{align*}
if membership of a pointed word in $\varphi$ depends only on its image under $h$. The following theorem, whose straightforward proof is omitted, generalizes to pointed word the classical equivalence of \mso and recognizable languages.
\begin{theorem}\label{thm:query-buchi} Let $\Sigma$ be a finite alphabet and let $X$ be a finite set of variables. A query   $\varphi \subseteq \queryalg X \Sigma$ is definable by an \mso formula with free variables $X$ if and only if it is recognized by a homomorphism into a finite query algebra. 
\end{theorem}
% \begin{proof}
%     A standard extension of compositionality for \mso.
%     %
%     % We only sketch the proof. In the proof sketch, we pay particular attention to an implicit semigroup in every query algebra, which is called the \emph{un-pointed semigroup}, and described below.
% %
%     % In the free query algebra $\queryalg X \Sigma$, there is a natural un-pointing  operation of type $\queryalg X \Sigma  \to \Sigma^+$ which keeps  the underlying word and forgets the distinguished positions. We can also define un-pointing an abstract query algebra $A$, as follows. 
%     % Define an equivalence relation $\sim$ on $A^+$ which identifies  two words $w_1, w_2 \in A^+$  if for every pointed word $w \in \queryalg X A$, and every appearance of $w_1$ as an infix of $w$ (such that no variables point to this infix), one can replace $w_1$ with $w_2$ without affecting the value of the multiplication operation of $A$. 
%     %  We write $\bar w$ for the equivalence class of a word $w \in A^+$ with respect to the equivalence relation $\sim$. One can easily show that (a) the equivalence relation $\sim$ is a  semigroup congruence; and (b) every equivalence class is of the form $\bar a$ for some one-letter word $a \in A$. This leads to the following definition: the \emph{un-pointed semigroup} of a query algebra  $A$ is the set $\bar A = \set{\bar a : a \in A}$, where the multiplication is the unique operation that turns $w \mapsto \bar w$ into a semigroup homomorphism.
% %
%     % Suppose that $A$ is query algebra. Define a \emph{unary polynomial} to be an element  $ p \in \queryalg X {(A+1)}$ where $+$ represents disjoint union and $1$ is a set with a single element that represents a placeholder. For a unary polynomial $p$, its underlying operation $p^A : A \to A$ is defined as follows: given input $a \in A$, replace every occurrence of  the placeholder of $p$ by $a$, giving an element of $\queryalg X A$, and then apply the multiplication operation. We say that a unary polynomial is \emph{un-pointed} if there is no occurrence of the placeholder that is pointed to by a variable. Define \emph{un-pointed equivalence}  in a query algebra $A$ to be the equivalence relation which identifies $a,b \in A$ if for every un-pointed unary polynomial $p$, both $a$ and $b$ have the same image under $p^A$. We write $\bar a$ for the equivalence class of $a \in A$ under un-pointed equivalence, and we write  $\bar A$ for the set of these  equivalences classes. One can easily show that $\bar A$ can be equipped with a semigroup operation
%     % % The homomorphism $h$ maps a word with a distinguished $Y$-tuple to the set of \mso formulas of rank $r$  
% \end{proof}



% One advantage that we get from describing query algebras in terms of monads, is that we automatically get some theorems that hold for all monads. One example is the existence of syntactic homomorphisms:  since the monad of queries is a finitary monad (for every choice of variables), it follows that for every query $\varphi$ there is a \emph{syntactic homomorphism}, which is a homomorphism that recognizes the query and uses the smallest possible algebra in the usual sense, see~\cite[Theorem 4.19]{bojanczyk_recobook}.






\paragraph*{An algebraic characterization of growth rate.} We now use the Seed Lemma and its proof to get  a characterization of homomorphisms of query algebras that recognize queries of growth rate with order $n^k$. The characterization is based on idempotents in a query algebra, which are defined as follows. We say that $e \in A$ is  \emph{idempotent}  if  for every partition 
\begin{align*}
X = X_1 \cup X_2
\end{align*}
and every pointed words $w_1 \in \queryalg {X_1} A$ and $w_2 \in \queryalg {X_2} A$, the following two pointed words in $\queryalg X A$ have the same value under the multiplication operation:
\begin{align*}
w_1 \cdot e \cdot w_2 \qquad 
w_1 \cdot e \cdot e \cdot w_2.\end{align*} In the above definition, we allow $X_i$ to be empty, in which case the pointed  word $w_i$ is also allowed to be empty.

 \begin{theorem}\label{thm:algebraic-growth-rate}
     Let $\varphi$ be a query that is recognized by a surjective homomorphism of query algebras
     \begin{align*}
     h : \queryalg X \Sigma \to A,
     \end{align*}
     with $A$ finite. Then $\varphi$ has growth rate of order at least $n^k$ if and only if:
     \begin{itemize}
         \item[(*)] there is some element in the image $h(\varphi) \subseteq A$  which can be obtained  applying the multiplication of the algebra  to a pointed word of the form 
         \begin{align*}
          \myunderbrace{\varlabel{Y_0}{a_0 }
         \cdot (\varlabel \emptyset {e_1} \cdot  \varlabel {X_1} {e_1
          } \cdot \varlabel \emptyset {e_1} )
          \cdot \varlabel{Y_1}{a_1 }
         \cdot (\varlabel \emptyset {e_2} \cdot  \varlabel {X_2} {e_2
          } \cdot \varlabel \emptyset {e_2} )
          \cdots 
          \varlabel{Y_{k-1}}{a_{k-1} }
         \cdot (\varlabel \emptyset {e_k} \cdot  \varlabel {X_k} {e_k
          } \cdot \varlabel \emptyset {e_k} )
          \cdot \varlabel{Y_k}{a_k }}{the index above each letter is the set of variables that point to it},
          \end{align*}
         such that $a_0,\ldots,a_k \in A$, the sets of variables $X_1,\ldots,X_k$ are all nonempty, and   $e_1,\ldots,e_k \in A$ are idempotent.
     \end{itemize}
     \end{theorem}
\begin{proof}
    Apply the Seed Lemma to the query. By the remarks at the end of the proof in Section~\ref{sec:proof-of-seed-lemma}, the Seed Lemma gives us an exact order $n^k$ of the growth rate, such that the lower bound is witnessed by a pattern as in Lemma~\ref{lem:sufficient-condition}. Such a pattern is the same thing as (*) in the present theorem. 
\end{proof}


==> mso.tex <==
%!TEX root = main.tex

\section{The hierarchies for growth rate and dimension coincide}
\label{sec:growth-dimension}
In this section, we recall the definition of string-to-string \mso interpretations. These are like the deterministic string-to-string \mso transductions of Engelfriet and Hogeboom~\cite[Section 4]{engelfrietMSODefinableString2001}, except that each output position is interpreted using a tuple of input positions, instead of a single position. In particular, the output size can be polynomial and not just linear.  


\paragraph{Monadic second-order logic on words.} We assume that the reader is familiar with the use of \mso to define properties of words; see~\cite[Section 2]{Thomas97} for an introduction to this topic.
The idea is to view a word as a model, whose universe consists of the positions in the word, and which is equipped with unary relations $a(x)$ for the labels and a binary relation $x \le y$ for the order on positions. We would like to underline the use of order $x \le y$ instead of successor  $x + 1 = y$. As far as the expressive power of \mso for  defining languages is concerned, there is no difference between the two choices, since the successor and order can be defined in terms of each other using \mso. However, for defining string-to-string functions the difference becomes important, since it might be possible to define a successor relation on $k$-tuples without being able to define the corresponding order, see ~\cite[p.~5]{msoInterpretations}. We use the model with order, which is more restrictive but behaves better (e.g.~the set of functions is closed under composition,
which is not true with the successor relation~\cite{msoInterpretations}).

\paragraph*{Interpretations.} The main topic of this paper is polyregular functions, which are a class of  string-to-string functions of polynomial growth. One of the several definitions is \mso interpretations, as described below. 
The basic idea behind an \mso interpretation of dimension $k \in \set{1,2,\ldots}$ is that it inputs a word, and creates an output word whose positions are some $k$-tuples of positions in the input word. (The model is deterministic, i.e.~it defines a string-to-string function, and not a binary relation on strings.) Which $k$-tuples are used, what is their order, and what are their labels -- all of this is described using \mso formulas. For example, the squaring function
\begin{align*}
w \mapsto w^{|w|}
\end{align*}
is defined by an \mso interpretation of dimension $k=2$, where the positions of the output word are all pairs $(x_1,x_2)$ of positions in the input word, the ordering is lexicographic, and the label is taken from $x_2$. This function has quadratic growth, which corresponds to the dimension. 



% Before giving a formal definition of \mso interpretations, we discuss a copying  feature of in the model. Consider the duplicating function
% \begin{align*}
% w \mapsto ww.
% \end{align*}
% There are two ways of defining this function. The first way uses a pre-processing step for copying: we first duplicate each input letter using the homomorphism that maps each letter $a$ to $aa$, and then we use an \mso interpretation of dimension $k=1$ to define the correct ordering on these letters (first we list all  even positions, followed by all odd positions). The second way avoids the pre-processing at the cost of a higher dimension $k=2$: we view positions of $ww$ as pairs $(x_1,x_2)$ of positions in $w$, such that $x_1$ is either the first or second position, and it  indicates whether or not the first or second copy of $w$ is used. (The second way works only for input words of at least two letters.) The advantage of the first way is that it uses optimal dimension $k=1$, while the advantage of the second way is that it avoids an extra copying construction in the syntax. Since this paper is concerned with the optimal dimension, we use the first way.

% \paragraph*{Formal definition of \mso interpretations.}

We now give a formal definition of \mso interpretations.  This definition includes an extra feature, called \emph{copying}: the idea is that output positions are described using $c \in \set{1,2,\ldots}$ copies of $k$-tuples of input positions (without copying, we would use $c=1$ copies). Copying makes the definition a bit cumbersome, and it could be removed without affecting the expressive power of the model, see~\cite[Footnote 1]{msoInterpretations}  or~\cite[Proof of Theorem 12]{lhote2020}. Nevertheless, removing the copying requires an increase in the dimension, which is something that  we care about in this paper. Therefore, we need the definition with copying.
\begin{definition}
    [\mso interpretation]
    An \emph{\mso interpretation} consists of the following ingredients:
\begin{enumerate}
    \item An input alphabet $\Sigma$ and an output alphabet $\Gamma$. Both alphabets are finite.
    \item A \emph{dimension} $k \in \set{1,2,\ldots}$ and a \emph{copying constant} $c \in \set{1,2,\ldots}$. The positions of the output string will be represented using $c$ copies of $k$-tuples of input positions, and therefore the output length will be at most $c \cdot n^k$.
    \item     For every output letter $a \in \Gamma$  and every $i \in \set{1,\ldots,c}$, a \emph{label formula}
    \begin{align*}
    \varphi^i_a(x_1,\ldots,x_k),
    \end{align*}
    which is an \mso formula over strings over the input alphabet. 
    This formula holds if the $i$-th copy of the $k$-tuple $(x_1,\ldots,x_k)$ represents an output position with label $a$. We require that for every $i$, every $k$-tuple is selected by at most one of the label formulas $\set{\varphi^i_a}_a$.
    \item For every $i,j \in \set{1,\ldots,c}$, an \emph{order formula}
    \begin{align*}
    \varphi^{i,j}_{\le}(x_1,\ldots,x_k,y_1,\ldots,y_k),
    \end{align*}
    which is an \mso formula over strings over the input alphabet. These formulas define the ordering of the copies of $k$-tuples which are positions of the output word. Therefore, in order for the \mso interpretation to be well-defined, these formulas need to define a total order on those copies of $k$-tuples of input positions which satisfy one of the label formulas.
    \item \label{it:distinguished-empty} A distinguished string in $\Gamma^*$ that will be used for the empty input string.
\end{enumerate}
The semantics of an \mso interpretation is a function $f \colon \Sigma^* \to \Gamma^*$ which maps a nonempty input string to the string obtained by using those  copies of $k$-tuples that are selected by the label formulas, and ordering them according to the order formulas. If the input string is empty, then the distinguished string from item~\ref{it:distinguished-empty} is used. 
\end{definition}

\tito{The notation $\Sigma^* \to \Gamma^*$ (rather than $\rightharpoonup$)
  suggests that we're working with \emph{total} functions throughout the paper.
  Maybe mention that explicitly + say that whether a family of formulas indeed
  specifies a total string-to-string function according to this definition is
  decidable by reduction to regular language emptiness? (I know it's obvious for
  people in the field, but it could be helpful for students)}

\tito{Suggestion: give two \mso interpretations of dimension 3 (extracted from the pebble transducer) and 2 (Mikołaj and Sandra's trick) for map power as running examples?}

% as follows. There are two parameters: the dimension $k \in \set{1,2,\ldots}$ and a copying constant $c \in \set{1,2,\ldots}$. It has an input alphabet $\Sigma$ and an output alphabet $\Gamma$; both alphabets are finite. For every output letter $a \in \Gamma$, there is corresponding \emph{label formula}, which is  an \mso formula 
% \begin{align*}
% \varphi_a(x_1,\ldots,x_k)
% \end{align*}
% that uses the vocabulary of words over alphabet $\Sigma$ and  specifies which $k$-tuples of positions in the input word will be used to produce an output position labelled by letter  $a$. We assume that for every input word, every $k$-tuple of positions is selected by at most one of the label  formulas.  Furthermore, there is an \emph{ordering formula}
% \begin{align*}
% \varphi_\le (x_1,\ldots,x_k,y_1,\ldots,y_k)
% \end{align*}
% which has the property that for every input word, the ordering formula defines a linear order on those $k$-tuples of positions which satisfy some label formula. The semantics of the interpretation is the function which inputs a word over the input alphabet, and outputs a word over the output alphabet whose positions  are those $k$-tuples of positions in the input word that satisfy some label formula, and the labels and  ordering of these positions given by the label and ordering formulas. 


% Define a \emph{non-copying \mso interpretation of dimension $k$} as follows. (The copying will be added and explained later on.) It has an input alphabet $\Sigma$ and an output alphabet $\Gamma$; both alphabets are finite. For every output letter $a \in \Gamma$, there is corresponding \emph{label formula}, which is  an \mso formula 
% \begin{align*}
% \varphi_a(x_1,\ldots,x_k)
% \end{align*}
% that uses the vocabulary of words over alphabet $\Sigma$ and  specifies which $k$-tuples of positions in the input word will be used to produce an output position labelled by letter  $a$. We assume that for every input word, every $k$-tuple of positions is selected by at most one of the label  formulas.  Furthermore, there is an \emph{ordering formula}
% \begin{align*}
% \varphi_\le (x_1,\ldots,x_k,y_1,\ldots,y_k)
% \end{align*}
% which has the property that for every input word, the ordering formula defines a linear order on those $k$-tuples of positions which satisfy some label formula. The semantics of the interpretation is the function which inputs a word over the input alphabet, and outputs a word over the output alphabet whose positions  are those $k$-tuples of positions in the input word that satisfy some label formula, and the labels and  ordering of these positions given by the label and ordering formulas. 

% If we are interested in the dimension of an interpretation, it will be important to extend the model with a copying feature, see~\cite[Footnote 1]{msoInterpretations} . To see the importance of copying, consider the duplicating function $w \mapsto ww$, which has linear size increase. This function increases the length, and thus it cannot be implemented by a non-copying \mso interpretation of dimension $k=1$. One workaround is to use a non-copying \mso interpretation of dimension $k=2$, by using the second coordinate to identify which copy is used (this workaround  works for inputs of at least two letters).  To avoid such unnecessary increase of the  dimension, we allow a pre-processing step which pads the input string  with separator symbols, as in the following example:
% \begin{align*}
%     \myunderbrace{abaa \quad \mapsto \quad \#\#a\#\#b\#\#a\#\#a\#\#}{this function is called 2-copying, because it inserts two copies of $\#$ }
%    \end{align*}
%    We can now define the central logical model of this paper:  a string-to-string function is an  \emph{\mso interpretation of dimension $k \in \set{1,2,\ldots}$} if it can be obtained by composing $c$-copying for some $c \in \set{0,1,\ldots}$ followed by a non-copying \mso interpretation of dimension $k$. The output size of such a function is easily seen to be of order at most $n^k$.

\paragraph*{Growth rate.}    We use the following terminology for the order of a function   $f \colon \Nat \to \Nat$:
\begin{align*}
\myunderbrace{f \in \Oo(n^k)}{order at most $n^k$}
\qquad 
\myunderbrace{n^k \in \Oo(f)}{order at least $n^k$}
\qquad 
\myunderbrace{f \in \Theta(n^k)}{order exactly $n^k$}.
\end{align*}
We are now ready to state one of our main results, which is that every  polyregular  function has growth rate of order exactly $n^k$ for some $k$, and it  can be defined by an \mso interpretation of dimension $k$.

\begin{theorem}\label{thm:optimization} For every polyregular function  $f \colon \Sigma^* \to \Gamma^*$ there exists some $k \in \set{0,1,\ldots}$ such that $f$ is an \mso interpretation of dimension $k$, and this dimension is optimal in the sense that the growth rate\footnote{Recall from the introduction that it is defined as $n \qquad \mapsto \max \set{|f(w)| : |w| \le n}$.} of $f$ has order exactly~$n^k$.
    % \begin{align*}
    % \myunderbrace{n \in \set{0,1,\ldots} \qquad \mapsto \qquad \max \set{|f(w)| : |w| \le n}}{this function is called the growth rate of $f$}.
    % \end{align*}
    \end{theorem}

\begin{remark}\label{rem:unary-output}
    In particular, the theorem rules out polyregular functions with growth rates such as $n^{2.5}$ or $n \cdot \log (n)$. Note that, since this property only depends on the output lengths, it suffices to consider the case of a unary output alphabet. Thus, the insight can also be deduced from the analogous property for marble transducers~\cite[Section~5]{Marble} since pebble and marble transducers compute the same functions with unary output~\cite[Corollary~18]{UnaryOutput}.
\end{remark}

Before proving the theorem, we remark that the construction is effective: the number $k$ and the  \mso interpretation of optimal dimension from the theorem can be computed given any of the effectively equivalent representations from~\cite{bojanczykPolyregularFunctions2018,msoInterpretations}, e.g.~an \mso interpretation of possibly sub-optimal dimension.

The theorem is going to be a direct consequence of a result on \mso queries that select tuples of positions in an input word, which is called the Seed Lemma and presented in the following section.


==> proof-of-seed.tex <==

 \subsection{Proof of the seed lemma}
 \label{sec:proof-of-seed-lemma}
 We now use the results from Sections~\ref{sec:semigroups} and~\ref{sec:factorization-forests}  to prove the Seed Lemma. Let $\varphi$ be a query that is recognized by a semigroup  homomorphism
 \begin{align*}
 h :  \Sigma^+ \to S.
 \end{align*}
 To this semigroup homomorphism, apply the Factorization Forest Theorem, yielding some upper bound $m \in \set{1,2,\ldots}$ on the height of factorization trees. For the rest of this proof, when talking  about factorization trees, we mean factorization trees for the homomorphism $h$. Also, a \emph{pointed factorization tree} will refer to such a  factorization tree, together with a distinguished tuple of positions indexed by the variables of the query.
  

One can show, see~\cite[Section 4]{bojanczykFactorizationForests2009}, that Factorization trees can be deterministically  computed by an \mso transduction in the following sense: there is a functional \mso transduction  which maps every input word $w \in \Sigma^+$ to some factorization tree  that has height at most $m$ and yield $w$. We use the name \emph{canonical factorization tree} for the output of this transduction. (The only properties of the canonical factorization tree that are interesting for us are that it is unique for each input word, and it can be computed in \mso.) Consider a skeleton $\tau$ obtained from pointed factorization tree (there are finitely many choices for $\tau$, since the height is bounded and the set of variables is fixed). Define $\varphi_\tau$
 to be the query with the same variables as $\varphi$, which  selects a pointed word if the corresponding leaves in the canonical factorization tree  have skeleton $\tau$. This is easily seen to be an \mso formula, because the canonical factorization is definable in \mso. By the Skeleton Lemma, we know that 
 \begin{align*}
 \varphi = \bigvee_{\tau \in I} \varphi_\tau
 \end{align*}
 for some  set  $I$ of skeletons, which is finite because there are finitely many possibilities for $\tau$.   To complete the proof of the Seed Lemma, we will show that the above decomposition satisfies the conclusions of the lemma, i.e.~for every $\tau \in I$  there is a subset of variables $Y \subseteq X$ which is a seed of $\varphi_\tau$, and  such  that $\varphi_\tau$ has growth rate of order at least $n^{|Y|}$.

 Fix a skeleton $\tau \in I$ for the rest of this proof. 
 Define  a \emph{movable interval} in the skeleton $\tau$ to be a maximal set of siblings that is closed under the ``linked sibling'' relation, and which does not contain a left-most or right-most sibling. 
 Here is a picture of a skeleton with all of its movable intervals:
 \mypic{13}
 A movable interval is contained in a set of at least 4 siblings, and therefore all of these siblings  are labelled by the same  semigroup element, which is an idempotent.
\label{page:segment}
  Define a \emph{segment} to be any set that is obtained by taking a movable interval, and adding all of its descendants.  Here is a picture of a skeleton with all of its segments distinguished: 
 \mypic{5}
  Since the movable intervals are pairwise disjoint, it follows that the  segments are laminar family, i.e.~every two segments  are disjoint or one is contained in the other. For each segment that is minimal inclusion-wise, choose  some variable that is captured by the segment, i.e.~the position pointed to by that variable is one of the leaves in the segment. Such a variable must exist,  because every node in the skeleton that is not a leftmost or rightmost sibling must have a descendant that is pointed to by a variable. Let $Y$ be the variables chosen this way, the number of these variables is the number of minimal segments. In the picture above, the two possible choices for $Y$ are $\set{x_1,x_4,x_5}$ and $\set{x_2,x_4,x_5}$.   We now prove that $Y$ is a seed, and the growth rate of $\varphi_\tau$ is of order at least $n^{|Y|}$. 
 
 \begin{itemize}
     \item \emph{$Y$ is a seed.}  Let $x$ be a variable of the query and choose $y \in Y$ so that its minimal segment (i.e.~the minimal segment that contains $y$) is contained in the minimal segment of $x$. By a straightforward analysis, we can see that in the skeleton $\tau$ one can from $y$ to $x$ by using a finite sequence of instructions from the following set:
     (a) go from a node to its parent;  (b) go  from a node to its previous linked sibling; (c) go  from a node to its next linked sibling;   (d) go  from a node to its leftmost child; or (e) go from a node to its rightmost child. Each of these instructions is deterministic, in the sense that the source node and the instruction name uniquely determines the target node. Therefore, in a pointed factorization tree, if we know the position of variable $y$, then we can uniquely determine the position of variable $x$ by following the sequence of instructions. Since the factorization tree that is used in the definition of the query $\tau$ is the canonical one and can therefore be computed in \mso, it follows that variable $x$ is uniquely determined by a variable $y$. 
     \item \emph{The growth rate is of order at least $n^{|Y|}$.} We use the sufficient condition from Lemma~\ref{lem:sufficient-condition}. Indeed, consider a mobile interval that corresponds to a minimal segment of the skeleton. As mentioned above, all siblings in this interval, and the missing part of the tree that corresponds to the dotted lines on either side of the interval, have the same idempotent value $e$ under the semigroup homomorphism, as explained in the following picture: 
     \mypic{8}
     In particular, the segment itself has a yield that is mapped to $e$. Therefore, if we take the minimal segments, which are pairwise disjoint, then we  get an instance of the pattern from Lemma~\ref{lem:sufficient-condition} that is a sufficient condition for growth of order at least $n^k$, where $k$ is the number of minimal segments. 
 \end{itemize}
 

The proof of Seed Lemma also shows that the sufficient condition from Lemma~\ref{lem:sufficient-condition} is also necessary, as we mentioned before. Indeed, we have shown that for each query $\varphi_i$ there is a seed $Y$ such that some tuple selected by $\varphi_i$ is an instance of the sufficient condition from Lemma~\ref{lem:sufficient-condition} with $k = |Y|$. Therefore, if we take $k$ to be the maximal size of the sets $Y$, ranging over queries $\varphi_i$, we can see that the growth rate is of order at most $n^k$, and there is an instance of the sufficient condition that implies order at least $n^k$. 


==> rubbish.tex <==
Consider a pebble transducer with atoms that has two pebbles. We assume without loss of generality that there is only one state of height zero, namely the initial one; every transducer can be easily modified so that it has this property, by directly moving between configurations with one pebble that would otherwise be separated by a configuration with zero pebbles. In this proof, as well as later in the paper, we will consider the tree structure of configurations. For a fixed input string, the \emph{tree of configurations} is the tree in which the nodes are configurations of the transducer which appear in the accepting run, not including the final configuration. The parent of a configuration in this tree defined to be the most recent configuration with a smaller stack of pebbles; the initial configuration is the root of the tree. The tree is sibling ordered, with the order on configurations corresponding to the order in which they appear in the run. The height of this tree is the maximal height of a pebble stack that appears in the run. In this particular proof, the height of the tree is two, since we consider transducer with two pebbles.


% For an input string, we view the set~\eqref{eq:range-pairs}
% as a directed graph in the following way. The vertices are pairs in the set, and the edge relation is the coordinate-wise order from the input string, i.e.~there is an edge from a pair to any other pair that is at least as big on both coordinates.
% We will produce this graph using an \mso interpretation, with the graph represented as a structure where the universe is the vertices, and which has a binary relation for the directed edge relation. 
% Without any assumptions on $\varphi$, this graph can be produced by an \mso interpretation of dimension $k=2$, where each vertex $(y,z)$ is represented by the corresponding pair of input positions. However,  if the  query $\varphi(x,y,z)$ satisfies the assumption of the lemma, then dimension $k=1$ would be enough, since the pairs can be represented using $N$ copies of the vertices $x$. 

% We know that for linear \mso interpretations which input strings (or, more generally, trees) and output graphs, the \emph{clique width} of the output graph has to be bounded, see~\cite[Theorem 3.1]{courcelle1995logical}. If the set~\eqref{eq:range-pairs} contains a $\ell \times \ell$ square, then the corresponding graph has an induced sub-graph which is the reflexive transitive closure of a directed  $\ell \times \ell$ grid as in the following picture 
% \mypic{27}
% Since square grid have unbounded cliquewidth, and cliquewidth can only decrease when taking induced sub-graphs, it follows that $\ell$ must be bounded. 

We begin by defining pebble transducers. This is a model of string-to-string transducer that is defined similarly to two-way automata, except that instead of having only a head, it has a stack of pebbles (with the topmost pebble   playing the role of the head) of bounded height.  The model was originally introduced for tree-to-tree transductions~\cite[Section 3.1]{DBLP:journals/jcss/MiloSV03}, but here we are interested in the string-to-string variant, which turns out to be one of the several equivalent characterizations of polyregular functions~\cite[Section 2]{bojanczykPolyregularFunctions2018}. 


In this paper, we use a variant of pebble transducers where the transitions are described by \mso formulas, i.e.~the successor configuration is from the current one by using \mso formulas.


A $k$-pebble transducer is defined as follows. There are finite input and output alphabets, and a finite set  of states, with each state having an associated height in $\set{0,1,\ldots,k}$.  A  \emph{configuration} of the transducer is defined to be a tuple which consists of an input string (a string over the input alphabet), a state, and a list of positions in the input string (called the \emph{pebble stack}) whose length is equal to the height of the state. Here is a picture of a configuration:
\mypic{21}  The topmost position in the pebble stack, $x_4$ in the picture above, is called the \emph{head} of the pebble stack. There is a  designated \emph{initial state} of height zero, which means that its pebble stack is empty. Finally, there is a \emph{configuration graph}, which is a directed graph where the vertices are configurations, and which has the following properties:
\begin{enumerate}
  \item {\bf Definability in \mso.} The edge relation is definable in \mso, in the following sense. For every two states $p$ and $q$, there is an  \mso formula 
  \begin{align*}
    \varphi(\myoverbrace{x_1,\ldots,x_i}{$i$ is height of\\ source state $p$},\myoverbrace{y_1,\ldots,y_j}{$j$ is height of\\ target state $q$})
    \end{align*}
    over the vocabulary of strings over the input alphabet such that two configurations with states $p$ and $q$ are connected by an edge if and only if they share the same input string, and the formula is true when the two pebble stacks are substituted for its free variables.
  \item {\bf Determinism.} Every configuration has at most one outgoing edge.
  \item {\bf Termination.} There are no infinite paths.
  \item {\bf Stack discipline.} If two  configurations are connected by an edge, then either: 
  \begin{enumerate}
    \item {\bf Push/pop.} One of the two pebble stacks is a prefix of the other; or 
    \item {\bf Move.} Two pebble stacks  have equal length, and agree on all pebbles except possibly the head.
  \end{enumerate}
 \end{enumerate}

 A \emph{run} of the pebble transducer is a path in the configuration graph; a run is called accepting if it begins in the initial state and ends in a configuration without outgoing edges (such configurations are called final). By determinism and termination, every input string admits a unique accepting run. To assign an output to each run, we assume that for each state there is a corresponding \emph{output string} over the output alphabet. The output of a run is obtained by concatenating the output strings of the states used in this run. The function computed by the transducer maps an input string to the  output of its unique accepting run.

This completes the definition of pebble transducers\footnote{As defined above, pebble transducers can use \mso formulas to go from one configuration to another, which will be usesful in our proofs. The classical model of pebble transducers is only allowed to move the head by one step and it can only ask local questions about the current configurations. The classical model  corresponds to the special case of our definition when the formulas defining the edges in the configuration graph are quantifier-free, using the vocabulary from Definition~\ref{def:ordered-representation} extended with constants for the first and last position, as well as functions for the successor and predecessor on positions.  Using the techniques of~\cite[Lemma 6]{engelfrietMSODefinableString2001}, one can show that our model is equivalent to the classical one, i.e.~for every pebble transducer in our model with \mso transitions, there is a pebble transducer that is equivalent (i.e.~it computes the same string-to-string function), has the same number of pebbles, and uses only quantifier-free formulas.  We do not present this proof here since it is not necessary for our results; this is because our results are lower bounds, and therefore they are made only stronger by allowing seemingly more powerful transition mechanisms. }. Although this might not be apparent at first glance, the syntax of pebble transducers is effective, which means that we can check if the \mso formulas that specify the edge relation satisfy the determinism, termination and stack discipline conditions. This is clear for determinism and stack discipline, by a reduction to satisfiability of \mso on finite strings.  For  termination, we use the following lemma, which crucially relies on stack discipline. (In the lemma below, we use the same notion of definability in \mso as when defining the transition relation.)

  \begin{lemma}\cite[Lemma 2.3]{bojanczykPolyregularFunctions2018}\label{lem:reachability-definable}
    The reachability relation in the graph of configurations is definable in \mso.
  \end{lemma}

  In particular, since there are finitely many configuration in every input string, termination is equivalent to saying that the configuration graph does not have any loop that is reachabile from an initial configuration, which can be decided using the above lemma.
  


\begin{lemma}
  For every $k$-pebble transducer, there is an equivalent $k$-pebble transducer (one that computes the same string-to-string function), in the all formulas are quantifier-free.
\end{lemma}

  A run is called \emph{accepting} if the first configuration uses the initial state and the last configuration uses the final state. The determinism and termination properties imply that for every input string, there is a unique accepting run. The \emph{output} of a run is defined to be concatenation of  the output strings of the configurations in the run.  
 
 
\begin{proof}[of Theorem~\ref{thm:deatomization}]
    By Lemma~\ref{lem:honest-done}, it is enough to show that if $\red f$ is computed by a $k$-pebble transducer, then it is computed by an honest $k$-pebble transducer. 

    Apply Lemma~\ref{lemma:brackets-no-popping}, yielding a $k$-pebble transducer  $\Aa$ that recognizes  $\red f$ and  satisfies the two items in  the conclusion of that lemma. 
    We now define  an honest $k$-pebble transducer that computes the same function. The honest transducer will use \mso queries in its transitions, which can be eliminated as shown in Claim~\ref{claim:add-mso-oracles}. 
    The honest transducer  enumerates through all of the configurations of $\Aa$, and for each one it does the following.  If the configuration has no output children -- which can be checked using an \mso oracle -- then no output is produced. Otherwise, suppose that   $q(\red w, \bar x)$ is a configuration of $\Aa$ that has at least one output child. Because the transducer satisfies  item 2 in  the conclusion of Lemma~\ref{lemma:brackets-no-popping}, this configuration is clean.   Apply Lemma~\ref{lem:almost-honest} to the state $q$ and the stack height $\ell$ of the configuration, yielding  a formula   $\varphi(\bar x, y)$ such that the output code block produced at configuration $q(\red w, \bar x)$ is equal to the infix of the input word that is  selected by the  positions $\set{y : \varphi(\bar x, y)}$.  We will simply output this infix, using the output instructions available to an honest pebble transducer. We consider two cases, depending on whether the height $\ell$ has the maximal value $k$ or not.
\begin{enumerate}
    \item If $\ell < k$, i.e.~the height is non-maximal, then the transducer can simply push another pebble, find the opening bracket of the code block $\set{y : \varphi(\bar x,y)}$, and then copy this code block to the output using the ``copy'' instruction. 
    \item The remaining case is when the height is maximal, i.e.~$\ell = k$. Because the transducer satisfies item  1 in the conclusion of Lemma~\ref{lemma:brackets-no-popping}, we know that all output children of $q(\red w, \bar x)$ will be reached by only moving the head, and not moving any of the pebbles at heights $< k$.  By the ``Futhermore'' part of the lemma,  with a number of exceptions that is at most some constant $m$, all head positions for the output children  will be in the set $\set{y : \varphi(\bar x,y)}$. If the size of this set is at most $m$, which can be checked using an \mso oracle, then the output code block is produced using a ``constant'' output instruction. Otherwise, if the set $\set{y: \varphi(\bar x, y)}$ has size bigger than $m$, then  at some point the head must enter this set. The honest simulating automaton refrains from outputting anything until the head enters this set, and upon first entering it, the code block is produced using the ``copy'' instruction.
\end{enumerate}
\end{proof}

    In the proof of this lemma, and other lemmas later on, it will be convenient to work with an extension of pebble transducers (with or without atoms) where \mso formulas are used for the transitions. 
    In this extension, instead of the usual transition relation, the successor relation on configurations is defined using \mso formulas, in the following sense. 
    
    In the rest of this proof we write configurations of a pebble transducer as $q(w,x_1,\ldots,x_\ell)$, where $q$ is the state, $w$ is the input word, and $x_1,\ldots,x_\ell$ are the pebbles (listed from the bottom of the stack to the top of the stack). Consider a binary relation on configurations, which only relates configurations with the same input word. We say that this binary relation is definable  in \mso if for every states $p$ and $q$ of the transducer, and stack heights $\ell, m \in \set{1,\ldots,k}$, there is an \mso formula $\varphi$ with $\ell+m$ free variables such that 
    \begin{align*}
    w \models \varphi(\myunderbrace{x_1,\ldots,x_\ell}{$\bar y$},\myunderbrace{y_1,\ldots,y_m}{$\bar y$}) 
    \end{align*}
    holds if and only if the relation is satisfied by the configurations $q(w,\bar x)$ and $p(w, \bar y)$. As usual, the formula $\varphi$ is allowed to talk about labels of positions and their order. In the case of configurations that involve atoms, i.e.~when talking about pebble transducers with atoms, the \mso formula is only allowed to ask if an input position stores an atom, but it is not allowed to ask which atom it is, or whether or not it is equal to an atom stored in some other position. 
    
    A pebble transducer with \mso transitions is defined in the same way as a usual pebble transducer, except that instead of giving a transition function, we give a binary relation on configurations that is definable in \mso. We require that the transition relation is (a) deterministic, which means that every configuration has a unique successor, unless it uses the accepting state; and (b) stack discipline is preserved, which means that the pebble stack in the target configuration is obtained from the pebble stack in the source configuration by either pushing some pebbles, or by moving the head, or by popping some pebbles. In item (b), when we talk about the head being moved, we do not require the head to be moved to a neighboring position. We use the name \emph{pebble transducer with \mso transitions} for this model, which comes in a version with atoms, and in a version without atoms.
    \begin{claim}\label{claim:add-mso-oracles} The same functions are computed by  $k$-pebble transducers as well as by $k$-pebble transducers with \mso transitions. This is  true with and without atoms.
    \end{claim}
    \begin{proof}
        The statement of the  claim in the case  of $k=1$ was shown by Engelfriet and Hoogeboom in~\cite[Theorem 7]{engelfrietMSODefinableString2001}. The case of $k > 1$ easily reduces to the case of $k=1$, since a $k$-pebble transducer can keep in its state the \mso theory, of appropriate quantifier rank, that corresponds to every part of the input string between two consecutive pebbles.
    \end{proof}

    Thanks to the above claim, to prove the lemma it will be enough to show that the function $f$ can be recognized by  a $k$-pebble transducer with atoms and \mso transitions. 



    
for every function  $
\alpha : \atoms \to \atoms$,
which is not necessarily a permutation. In the diagram, $\alpha$ is extended to strings in the natural way, without changing the letters from $\Sigma$ or $\Gamma$.


We will care only about functions which are \emph{atom-oblivious}, which means that the function commutes with every function of type $\atoms \to \atoms$ (extended in the obvious way to input and output strings of the function of $f$). The general idea behind atom-oblivious functions is that they are allowed to copy the input atoms to the output, but they are not allowed to ask any questions about them. Also, an atom-oblivious function is uniquely defined by its outputs for those inputs where every atom appears at most once.

\begin{myexample}
In this example, we compare atom-obliviousness with the notion of \emph{equivariance} from sets with atoms, which is the weaker requirement that a function commutes with all functions of type $\atoms \to \atoms$ that are permutations.  Consider functions  of type $\atoms^* \to \atoms^*$. The identity function, the reverse function, and the duplicating function $w \mapsto ww$ are all atom-oblivious (and therefore also equivariant). Here is a function that is equivariant but not atom-oblivious. If  the first two letters of the input word are defined and  different, then the function returns  the input, otherwise the function returns the  empty word. This function is not atom-oblivious, because if $\alpha$ is the function that maps all atoms to $1$, then we have 
\begin{align*}
\alpha(f(12)) = \alpha(12) = 11 \neq \varepsilon = f(11) = f(\alpha(12)).
\end{align*}
\end{myexample}

Consider a function $f$ as in~\eqref{eq:atom-transducer-type}.
We will  simulate  $f$ by a function that uses  finite alphabets, by representing each atom as a string of the following form:  an opening bracket, followed by a string over a unary alphabet $\set a$, followed by a closing bracket. 
We use the name \emph{code block} for strings of this form, i.e.~strings of the form $\langle a^* \rangle$. We assume that the letter $a$ as well as both brackets $\langle$ and $\rangle$  are fresh, in the sense that they are  disjoint with the alphabets $\Sigma$ and $\Gamma$ used by $f$.
Define an \emph{atom representation} to be any function which maps atoms to code blocks (we will be most interested in atom representations that are injective, but injectivity is not always required). Throughout this section, we use a colour convention where the colour red is used for strings to which an atom representation has been applied, i.e.~red variables denote words where atoms are represented using code blocks.


Define a  \emph{de-atomization} of the function $f$ to be any function $\red f$ (here we use the colour convention where the red font indicates that code blocks are used instead of atoms) which makes the following diagram  commute for every atom representation $\alpha$:
\[
\begin{tikzcd}[column sep=3cm]
(\Sigma + \atoms)^*
\ar[r,"f"]
\ar[d," \alpha"'] &
(\Gamma + \atoms)^*
\ar[d," \alpha"]\\
(\Sigma + \langle a^* \rangle)^* 
\ar[r,red,"\red f"']&
(\Gamma + \langle a^* \rangle)^*
\end{tikzcd}
\]
 In the above diagram, the atom representation is extended in the obvious way to strings that mix atoms with other letters.  It is not hard to see that if $f$ atom-oblivious, then it has a unique de-atomization. 
This de-atomization works as follows: given an input string for the de-atomization,  replace every code block by a distinct atom (if the same code block has several occurrences, a different atom is used for each occurrence), then apply $f$, and finally  replace each atom  by the corresponding  code block. If the function is atom-oblivious, then the output of the de-atomization defined above  does not depend on the choice of atoms used to replace  code blocks. 


The height of a node in a tree is defined to be the height of its subtree. Leaves have height zero, and the height of the root is the height of the entire tree.  The height of a configuration of the pebble automaton is defined to be its height in the tree of configurations. Without loss of generality we assume that the transducer is such that  every output position is produced with a full stack, and that the tree of configurations is balanced. These additional assumptions can be assumed without loss of generality, in the sense that for every pebble transducer there is another pebble transducer which computes the same function, has the same number of pebbles, and which a satisfies the additional assumptions. Because the tree of configurations is balanced, every configuration $c$ satisfies 
\begin{align*}
\text{(height of $c$)} + \text{(number of pebbles in $c$)}  = \text{number of pebbles in transducer}
\end{align*}





The proof is by contradiction. The main step is given in the following lemma, which describes outputs of a 2-pebble transducer on input strings that use each atom at most once. The idea is that the output string can be decomposed into a linear number of factors, such that in each of the factors every atom (with at most one exception) appears a constant number of times.

\begin{lemma}\label{lem:two-pebble-outputs}
    Consider a function $f$ that is recognized by a $2$-pebble transducer with atoms. There exists a constant $c \in \set{1,2,\ldots}$ such that for every input string $w$ where every atom appears once, one can find a decomposition of the output string 
    \begin{align*}
    f(w) = v_1 \cdots v_m
    \end{align*}
    such that: (1) in each of the strings $v_1,\ldots,v_n$, every atom appears at most $c$ times; and (2) the number $n$ of strings is at most $n$ times longer larger than the length of $w$.
\end{lemma}
\begin{proof}
    Each string $v_i$ corresponds to the part of the output string  that is output when pebble 1 was in a given position. 
\end{proof}

We now complete the proof of Theorem~\ref{thm:two-pebble-counter-example-atoms}, by showing that the map power function is incompatible with Lemma~\ref{lem:two-pebble-outputs}. Indeed, apply the lemma to a hypothetical 2-pebble transducer with atoms that recognizes the map power function, yielding a constant $c$. Consider an input  string of the form 
\begin{align*}
w = w_1 | \cdots | w_{n}
\end{align*}
where every atom appears at most once, and every  word $w_i$ has two atoms. The length of the output string
\begin{align*}
    (w_1)^n \cdots (w_n)^n
\end{align*}
is quadratic in $n$.  Consider a factorization $v_1 \cdots v_m$  as obtained from Lemma~\ref{lem:two-pebble-outputs}. By condition (1) of the lemma, each of the strings $v_1,\ldots,v_m$ can have at most constant length (in terms of $c$), since otherwise it would contain some atom more than $c$ times. By condition (2), the number $m$ of strings is linear in $n$. Therefore, the size of the output must be at most linear, a contradiction. 
\subsubsection{Zebras with atoms}
\label{sec:zebras}

Define the $k$-zebra function with atoms in the same way as the $k$-zebra function, except that $\atoms$ is used instead of $\set{a,b}$. 

\begin{theorem}\label{thm:no-zebra-atoms}
    The $k$-zebra function with atoms cannot be recognized by any pebble transducer with atoms that has less than $2k$ pebbles.
\end{theorem}
\begin{proof}
    (fill in)
A direct adaptation of the technique for map power will not work, since it is based on $k=2$ pebbles. 
\end{proof}


\begin{lemma} Consider a pebble transducer $\Aa$ which computes the $2k$-zebra function. If $\rho$ is a reachable run of order $\ell$, and the input tree is wide enough, then   all subtrees of the output of $\rho$ have height at most $\ell$.
\end{lemma}

\begin{lemma}\label{lem:zebra-lower-bound-technical}
Let $\Aa$ be a pebble transducer which computes the $2k$-zebra function. 
For every $\ell \in \set{1,2,\ldots, 2k}$ there exist constants $K(\ell)$ and $W(\ell)$ such that  if $\rho$ is a reachable run of order $\ell$ over some input tree of height $k$ and width at least $W(\ell)$, and  $f_\ell(t,x,y)$ is a subtree of the output of $\rho$, then both $x$ and $y$ can be defined from the first configuration of $\rho$ using \mso formulas of size at most $K(\ell)$.
\end{lemma}

\begin{proof} Suppose that the $2k$-zebra function is computed by some transducer with $\ell < 2k$ pebbles. Let $\rho$ be the entire run of this transducer over some   sufficiently wide input tree $t$. By Lemma~\ref{lem:zebra-lower-bound-technical}, every subtree of the output that has height $\ell$ is of the form $f_\ell(t,x,y)$ for some nodes $x$  and $y$ which can be defined, based on the initial configuration of the transducer, using \mso formulas of  at most constant size $K(\ell)$. The number of such nodes is also constant, and therefore if the width of the tree is sufficiently large, then the width will be greater than the number of subtrees of the output that have height $\ell$. On the other hand, if $\ell < 2k$, then the number of subtrees of height $\ell$ must be at least the width, a contradiction.
\end{proof}


\begin{proof}[of Lemma~\ref{lem:zebra-lower-bound-technical}]
Induction on $\ell$. Consider a configuration $c$ of order $\ell+1$, whose stack of pebbles is 
\begin{align*}
\myunderbrace{z_m, z_{m-1},  \ldots, z_{\ell+1}}{
    $\bar z$
}
\end{align*}
and let $\rho$ be the run of order $\ell$ that is between the configuration $c$ and the next configuration of order $\ell+1$ (or the end of the run). Every pebble stack that will appear in the run $\rho$ is of the form $\bar z z_\ell$ for some node $z_\ell$ which corresponds to the pebble of order $\ell$. 
\begin{claim}
    There is a finite set $\Phi$ of \mso formulas, which depends only on the transducer and $\ell$, with the following property. Each of these formulas is a relation on $m+2$ nodes, which is functional from the first $m$ arguments to the last two arguments. Furthermore, 
\end{claim}
\begin{align*}
m = \text{number of pebbles in the transducer} + 1 - \ell.
\end{align*}
This number is chosen so that in a configuration of order $\ell$, the number of pebbles is $m$. Let
\begin{align*}
\myunderbrace{z_{m+\ell}, z_{m+\ell-1},\ldots,z_{\ell}}{}
\end{align*}
$z_1,\ldots,z_m$ be the pebble stack in the first configuration of the run $\rho$. 


For an input tree $t$ with a pair of distinguished nodes $(x,y)$, define its $\ell$-critical configuration to be  the most recent configuration of order $\ell$ that appeared in the run of the pebble transducer before starting  the output of the tree
\begin{align*}
f(t,x,y).
\end{align*}
The function that maps $(t,x,y)$ to its $\ell$-critical configuration is definable in \mso. Define the $\ell$-critical node of $(x,y)$ to be the position of the pebble of order $\ell$ in the corresponding $\ell$-critical configuration. 

\begin{claim}
    There is a finite set of \mso formulas, which are 
\end{claim}

We will show that there is a constant $K$ such that for every pair of nodes $(x,y)$ in an input tree, there are at most $K$ children $x'$ of $x$ such that $f(t,y,x')$ is produced in the run $\rho$. 



We have a large number $n$ of consecutive siblings 
\begin{align*}
x_1,\ldots,x_n
\end{align*}
of some node $x$, and some other node $y$ such that the transducer outputs all of the trees 
\begin{align*}
f_\ell(y,x_1), \ldots,f_\ell(y,x_n).
\end{align*}
Let $y_1,\ldots,y_m$ be all of the children of $y$. We know that there is a finite set of \mso formulas such that $X \times Y$ is the 

\begin{claim}There is an \mso query $\varphi$ of arity $m+2$ such that 
    \begin{enumerate}
        \item there is some bound $N$ such that for every input tree $t$ and every $m$-tuple of nodes $\bar z$, there are at most $N$ pairs $(x,y)$ which satisfy $\varphi(\bar z, x,y)$.
        \item if $t$ is an input tree and 
        $f(t,x,y) $ of height $\ell-1$  $\ell$-subcomputation  order $\ell$-subcomputation with parameters $\bar z$, then there is some node $z$ such that $\varphi(\bar z, z, x, y)$
    \end{enumerate}
    \end{claim}



\begin{claim}There is an \mso query $\varphi$ of arity $m+2$ such that 
    \begin{enumerate}
        \item there is some bound $N$ such that for every input tree $t$ and every $m$-tuple of nodes $\bar z$, there are at most $N$ pairs $(x,y)$ which satisfy $\varphi(\bar z, x,y)$.
        \item if $t$ is an input tree and 
        \begin{align*}
        f(t,x,y) 
        \end{align*}
        is an output tree that is output during the order $\ell$-subcomputation with parameters $\bar z$, then there is some node $z$ such that $\varphi(\bar z, z, x, y)$
    \end{enumerate}
    \end{claim}
\begin{proof}
    
\end{proof}




We assume that the reader is familiar with the basic notions of logic. We use the name \emph{vocabulary} for a set of relation names with associated arities, and a model over a vocabulary is defined to be an underlying set (called the \emph{universe} of the model), together with an interpretation of each relation name as a relation on the universe. To define properties of such models, we use monadic second-order logic \mso. 


Define an \emph{\mso interpretation} to be a transformation on models that is a composition of two types of transformation described below: first we apply a  \emph{copying transformation}, and then we apply a \emph{non-copying \mso interpretation}.

\begin{enumerate}
    \item For a vocabulary $\tau$ and copying constant $c \in \set{1,2,\ldots}$, define the \emph{copying} operation to be a function that inputs a model  over vocabulary $\tau$, and outputs a model which consists of $c$ disjoint copies of the input model (these copies are ordered, i.e.~there is a first copy, second copy, etc.), equipped with an extra $c$-ary relation that is interpreted as the set of tuples that can be obtained by taking some $a$ in the input model, and listing all their copies in the correct order. 
    \item A  \emph{non-copying \mso interpretation} with input vocabulary $\tau$ and output vocabulary $\sigma$ is given by a number $k \in \set{1,2,\ldots}$ called the \emph{dimension},  a \emph{universe formula}, and a family of \emph{relation formulas} formulas $\set{\varphi_R}_{R \in \sigma}$ indexed by relations in the output vocabulary. All of the formulas are \mso formulas where all  free variables are all first-order variables.  The universe formula has  $k$ free  variables, and a relation formula $\varphi_R$ has $k$ times as many free variables as  the arity of the relation $R$. The semantics of the interpretation is a function from models over the input vocabulary to models over the output vocabulary. If the input model is $\mathfrak A$, then the output model is defined as follows: its universe is the $k$-tuples of elements in $\mathfrak A$ that satisfy the universe formula, while an $n$-ary relation $R$ of the output vocabulary is interpreted as those $n$-tuples of $k$-tuples (which can be viewed as $(n \cdot k)$-tuples) that satisfy the relation formula $\varphi_R$.
\end{enumerate}
If the input structure has a finite universe of size $n$, and we apply copying with constant $c$ followed by a non-copying \mso interpretation of dimension $k$, then the output model will have size at most $(c \cdot n)^k$, in particular of polynomial size. Unlike first-order interpretations, \mso interpretations are not in general closed under composition.  However, the situation changes if we consider \mso interpretations that input and output strings. We say that a function $f : \Sigma^* \to \Gamma^*$ is an \mso interpretation of dimension $k$ if there is some \mso interpretation of dimension $k$, such that for every nonempty input word $w \in \Sigma^+$, applying the interpretation to the model of $w$ yields the model of $f(w)$. This definition does not consider the empty input word, and therefore to fully specify $f$ one needs to give the interpretation plus the output of $f$ on the empty word. 

\subsection{The upper bound}
\label{sec:seed-lemma}

In this section, we prove the upper bound  from Theorem~\ref{thm:algebraic-growth-rate}. We show that there is some $k \in \set{0,1,\ldots}$ such that the query $\varphi$ can be decomposed as a finite union 
\begin{align*}
\varphi = \bigvee_{i \in I} \varphi_i,
\end{align*}
such that for every $i \in I$, there is some $k_i \in \set{0,1,\ldots}$ such that $\varphi_i$ has a seed of $k_i$ variables (and hence the growth rate of $\varphi_i$ is at most $n^{k_i}$), and the image $h(\varphi_i)$ contains some element of the algebra that has degree at least $k_i$ (and hence the growth rate of $\varphi_i$ is at least $\lambda_i \cdot n^{k_i}$ for some $0 < \lambda_i \le 1$). In particular, the growth rate of $\varphi_i$ is exactly $\Theta(n^{k_i})$, and Theorem~\ref{thm:algebraic-growth-rate} follows by taking $k$ to be the maximum of $\set{k_i}_i$. In the proof, we use  the Factorization Forest Theorem, which is described below. 




\begin{definition}
    [Query algebra] Let $X$ be a finite set of variables. A query algebra over variables $X$ consists of an underlying set $A$ equipped with the following operations:
    \begin{enumerate}
        \item A \emph{variable operation} $var : A \to \powerset X$. The idea is that an element of variables $Y \subseteq X$ represents a word with a distinguished $Y$-tuple of positions.
        \item A partial binary \emph{concatenation  operation}  of type $A^2 \to A$, written multiplicatively as $a \cdot b$, and satisfying the following axioms: 
        \begin{eqnarray}
            a \cdot b \text{ is defined} & \iff & var(a) \cap var(b) = \emptyset \\
            var(a \cdot b) &=& var(a)\cup var(b)\\
            (a \cdot b) \cdot c &=& a \cdot (b \cdot c).
        \end{eqnarray}
        In particular, the variable-free elements of $A$, i.e.~those which have an empty set variables, form a semigroup.
        \item A  \emph{variable elimination} operation of type $A \to A$, which maps every element $a \in A$ to a variable-free  element denoted by $\bar a \in A$, subject to the axiom:
        \begin{align}
            \overline{a \cdot b}  = \overline a \cdot \overline b.
        \end{align}
    \end{enumerate}
\end{definition}


For an alphabet $\Sigma$ and a set of variables $X$, the \emph{free query algebra} $\queryalg X \Sigma$ is defined to be the query algebra where the underlying set is words in $\Sigma^*$ with distinguished tuples of positions that are indexed by subsets $Y \subseteq X$; and where the structure of the query algebra is defined in the natural way.
 
A \emph{homomorphism} of two query algebras over the same set of variables is a function between the underlying sets that is compatible with all three operations of query algebras: the variable operation, concatenation, and variable elimination. As far as this paper is concerned,  the purpose of query algebras is to recognize \mso queries using finite query algebras. Here, an \mso query  with free variables $X$ and input alphabet $\Sigma$ can be seen as a subset of the free query algebra $\queryalg X \Sigma$, which only contains elements whose variables are the full set of variables $X$. 

==> seed-lemma.tex <==
%!TEX root = main.tex

\subsection{The growth rate of queries}
\label{sec:seed-lemma}
This section describes  the Seed Lemma, which explains the growth rate of \mso  queries, i.e.~\mso formulas with free variables that are used to select tuples of distinguished positions in an input word. Theorem~\ref{thm:optimization} about the growth rate of polyregular functions will follow immediately from the  Seed Lemma. 

We use tuples of positions that are indexed by some set $X$ of free variables, such tuples are called  $X$-tuples. For a query with free variables $X$, we will be interested in the order of  its \emph{growth rate}, which is the function 
\begin{align*}
n \in \set{1,2,\ldots} \quad \mapsto \quad \max_{|w| \le n}. \ \text{number of $X$-tuples selected in $w$}.
\end{align*}

 Here are some examples of queries over variables $\set{x_1,x_2,x_3}$ and the orders of their growth rates:
\begin{align}\label{eq:query-examples}
\myunderbrace{x_1 < x_2 < x_3}{a query with growth \\ \scriptsize rate of order $n^3$}
\qquad 
\myunderbrace{x_1 < x_2\ \land\  x_2+1 = x_3}{a query with growth \\ \scriptsize rate of order $n^2$}.
\end{align}
If a query has $k$ free variables, then its growth rate is at most $n^k$, however  smaller growth rates are possible because of  dependencies between variables. The Seed Lemma in this section explains  these dependencies in more detail.

A simple kind of dependency is when a query with variables $X$ admits a subset  $Y \subseteq X$ which  determines all variables, in the following sense:  for every input word and every  $Y$-tuple of positions, there is at most one  extension to an $X$-tuple of positions that satisfies $\varphi$.  Such a subset of the variables is called a \emph{seed}; it is the same thing as a key in databases.  For example, in the second query~\eqref{eq:query-examples}, the subset $\set{x_1,x_2} \subseteq \set{x_1,x_2,x_3}$ is a seed, because variable $x_3$ is uniquely determined by variable $x_2$. The size of a seed provides a tighter upper bound on the growth rate, as compared to the number of variables:  if  a query has a seed of at most $k$ variables, then it can select at most $n^k$ tuples in an input word of length $n$. The main result of this section is the following lemma, which shows that every query can be decomposed into a finite disjunction of queries where the upper bounds provided by the seed sizes are tight.

\begin{lemma}[Seed Lemma]
    Every \mso query $\varphi$ can be decomposed as a finite disjunction 
    \begin{align*}
    \varphi = \bigvee_{i \in I}\varphi_i
    \end{align*}
    such that for every $i \in I$ there is some $k_i \in \set{0,1,\ldots}$ such that: (a) $\varphi_i$ has a seed of at most $k_i$ variables; and (b) $\varphi_i$ has  growth rate of order at least $n^{k_i}$.
\end{lemma}

Before proving the Seed Lemma, we show how it implies Theorem~\ref{thm:optimization}. 

\begin{proof}[of Theorem~\ref{thm:optimization}]
    Consider a polyregular function $f$, given as an \mso interpretation. We can assume without loss of generality that this is a non-copying \mso interpretation; this might require increasing the dimension, which will be anyway optimized in our construction. 
     Let $\ell$ be the dimension -- possibly sub-optimal -- of this interpretation, and let $\varphi(x_1,\ldots,x_\ell)$ be the disjunction of all the label formulas in the interpretation. The growth rate of the polynomial function is the same as the growth rate of the query $\varphi$.   Apply the Seed Lemma to this formula $\varphi$, yielding a growth rate of order $n^k$ and a decomposition 
    \begin{align*}
    \varphi(x_1,\ldots,x_\ell) = \bigvee_{i \in I} \varphi_i(x_1,\ldots,x_\ell),
    \end{align*}
    such that each query $\varphi_i$ has a seed of at most $k$ variables. 
    It remains to show that $f$ can be defined by an \mso interpretation of dimension $k$. The idea is simple: the new \mso interpretation (of optimal dimension $k$) uses the seeds, and extends them to $\ell$-tuples (of possibly larger sub-optimal dimension) that were used by the original \mso interpretation.  The order on the seeds is obtained by considering their unique expansions to $\ell$-tuples, and applying the order from the original \mso interpretation. Likewise we define the labels for the seeds.  Note that we needs several copies of each $k$-tuple, namely one for each disjunct $\varphi_i$, and hence we need the copying feature of \mso interpretations.
\end{proof}

The rest of this section is devoted to proving the Seed Lemma.  In Section~\ref{sec:semigroups}, we introduce some semigroup terminology for recognizing queries, which is then used to define   a sufficient condition for growth rate of order at least $n^k$.  In Section~\ref{sec:factorization-forests}, we recall the Factorization Forest Theorem. In Section~\ref{sec:proof-of-seed-lemma}, we use the Factorization Forest Theorem and the sufficient condition to complete the proof of the Seed Lemma. 


\input{semigroups}
\input{factorization-forests}
\input{proof-of-seed}

==> semigroups.tex <==
\subsection{Semigroups recognizing queries}
\label{sec:semigroups}
We begin by describing  how queries can be recognized using homomorphisms into finite semigroups, and we identify a pumping pattern in such homomorphisms that is sufficient for growth of order at least $n^k$.  

\paragraph*{Pointed words and queries.}   A \emph{pointed word} is defined to be a word, called the \emph{input word}, together with a distinguished tuple of positions that is indexed by some finite set of variables.  
  We allow the  input word to be empty, but this is only possible if the variable set is empty, since each variable must point to some position. Pointed words with disjoint sets of variables can be concatenated:  if $w_1$ is a pointed word with variables $X_1$ and $w_2$ is a pointed word with variables $X_2$, and these two sets of variables are disjoint,  then $w_1 \cdot w_2$ is a pointed word with variables $X_1 \cup X_2$. 
 
 A \emph{query with variables $X$ and input alphabet $\Sigma$} is defined to be any set of pointed words where the input word uses alphabet $\Sigma$ and the variables are $X$.
We are  interested in queries which can be defined in \mso, i.e.~they can be defined by an \mso formula where the set of  free variables is $X$, and all of these variables are first-order variables (i.e.~there are no free second-order variables). The vocabulary used by the formula is the usual one for \mso over words: it has unary predicates for the labels of positions, and a binary predicate for the order on positions. For example, the query 
\begin{align*}
\varphi(x,y) = \exists z \ x < z \land z < y
\end{align*}
with variables $\set{x,y}$ selects pointed words where $x < y-1$. This is a first-order query, but we could use \mso to say that the distance between $x$ and $y$ is even.


% This approach to recognizability is tailored to be as lightweight as possible so that it is still sufficient to prove the Key Lemma. In Section~\ref{sec:monad} we recast the results from this section using a  more principled algebraic approach.
\paragraph*{Semigroups.} Recall that a \emph{semigroup} is a set equipped with an associative binary operation, and a \emph{semigroup homomorphism} is a function between two semigroups that is compatible with the semigroup operation. 
We say that a query $\varphi$ with input alphabet $\Sigma$ is \emph{recognized} by a semigroup homomorphism
\begin{align*}
h : \Sigma^+ \to S
\end{align*}
if for every pointed word, membership in the query is not changed if we replace an un-pointed infix (an infix of the input word without any variables pointing to it) with another un-pointed infix of same value under $h$. In other words, for every un-pointed words $w,w'$, and  every pointed words $w_1,w_2$ whose variables form a partition of the variables of the query, we have 
\begin{align*}
h(w)=h(w') \quad \text{implies} \quad w_1 \cdot w \cdot w_2 \in \varphi \iff w_1 \cdot w' \cdot w_2 \in \varphi.
\end{align*}
In the above, either of the two pointed words $w_1$ or $w_2$ could be empty, if its set of variables is empty.
The following folklore lemma is an extension to queries of the usual correspondence between \mso and recognizable languages.
\begin{lemma}
    \label{lem:compositionality} A query is definable in \mso if and only if it is recognized by a homomorphism into a finite semigroup.
\end{lemma}
\begin{proof}
    The result is a standard application of compositionality of \mso, see~\cite[Section 2.1]{bojanczyk_recobook}, adapted from words to pointed words.
    Since the adaptation  is very standard, we only sketch it. 
    For the right-to-left implication, we observe that for every homomorphism into a finite semigroup, an \mso formula can compute the value of the homomorphism on any infix between two consecutive variables.  For the left-to-right implication, we use  compositionality of \mso to conclude that  the truth value of a query is not affected if an un-pointed interval is replaced by some other un-pointed interval with the same  \mso theory of suitable  quantifier rank, and the function that computes this \mso theory is a semigroup homomorphism.
\end{proof}




\paragraph*{A sufficient condition for growth of order at least $n^k$.}   Recall  that an \emph{idempotent} in a semigroup is an element $e$ that satisfies $e \cdot e = e$. Idempotents are usually used to describe some form of pumping, and the following lemma is no exception. 


\begin{lemma}
    \label{lem:sufficient-condition} Let $\varphi$ be a query that is recognized by a semigroup homomorphism $h : \Sigma^+ \to S$ with $S$ finite. The following condition is sufficient for a growth rate of order at least $n^k$: the query selects some pointed word 
    \begin{align*}
    w_0 \cdot 
    (e_1 \cdot v_1 \cdot e_1) \cdot w_1 \cdot
    (e_2 \cdot v_2 \cdot e_2) \cdot w_2 \cdots
    (e_k \cdot v_k \cdot e_k) \cdot w_k
    \end{align*}
    where $w_0,\ldots,w_k$ and $e_1,v_1,\ldots,e_k,v_k$ are pointed words such that $v_1,\ldots,v_k$ all have nonempty variables, each $e_i$ is obtained from $v_i$  by removing all variables, and each $e_i$ is mapped by $h$ to an  idempotent of the semigroup $S$.
\end{lemma}
\begin{proof}
For $n \in \set{1,2,\ldots}$, consider  the following pointed word
        \begin{align*}
            w_0 \cdot e_1^n \cdot w_1 \cdot e_2^n \cdot  w_2 \cdots e_k^n \cdot w_k
            \end{align*}
            which is missing the variables used by $v_1,\ldots,v_k$. 
    The length of this word is linear in $n$, since $k$ is assumed to be fixed. The lemma will follow from the fact that  there are at least $(n-2)^k$ ways of choosing the distinguished positions in this word  so that the resulting pointed word  is selected by the query. This is done by choosing for  each  $i \in \set{1,\ldots,k}$ one of the $n-2$ copies of $e_i$ inside $e_i^n$ that are not the first or last copy, and placing the variables inside that copy in a way that creates the pointed word $w_i$.  Since $e_i$ is mapped by $h$ to an idempotent, all earlier copies and also all later copies will be mapped to this same idempotent.
\end{proof}

From the proof of the Seed Lemma that will be presented later in this section, it will follow that the condition in the above lemma is also necessary.
